Knot Floer homology as immersed curves

To a nullhomologous knot $K$ in a 3-manifold $Y$, knot Floer homology associates a bigraded chain complex over $\mathbb{F}[U,V]$ as well as a collection of flip maps; we show that this data can be interpretted as a collection of decorated immersed curves in the marked torus. This is inspired by earlier work of the author with Rasmussen and Watson, showing that bordered Heegaard Floer invariants $\widehat{\mathit{CFD}}$ of manifolds with torus boundary can be interpreted in a similar way. Indeed, if we restrict the construction in this paper to the $UV = 0$ truncation of the knot Floer complex for knots in $S^3$ with $\mathbb{Z}/2\mathbb{Z}$ coefficients, which is equivalent to $\widehat{\mathit{CFD}}$ of the knot complement, we get precisely those curves; this paper then provides an entirely bordered-free treatment of those curves in the case of knot complements, which may appeal to readers unfamiliar with bordered Floer homology. On the other hand, the knot Floer complex is a stronger invariant than $\widehat{\mathit{CFD}}$ of the complement, capturing "minus" information while $\widehat{\mathit{CFD}}$ is only a "hat" flavor invariant. We show that this extra information is realized by adding an additional decoration, a bounding chain, to the immersed multicurves. We also give geometric surgery formulas, showing that $HF^-$ of rational surgeries on nullhomologous knots and the knot Floer complex of dual knots in integer surgeries can be computed by taking Floer homology of the appropriate decorated curves in the marked torus. A section of the paper is devoted to a giving a combinatorial construction of Floer homology of Lagrangians with bounding chains in marked surfaces, which may be of independent interest.

==> sections/old.tex <==
% !TEX root = ../CFKcurves.tex
%old.tex

The main aim of this paper is to show that the algebraic objects arising in knot Floer homology, namely collections of bigraded complexes along with collections of flip isomorphisms, are equivalent to collections of immersed multicurves with bounding chains in certain infinite marked cylinders. In this section we discuss the easy direction of that equivalence, showing that any immersed multicurve with bounding chain in such a surface determines a collection of bigraded complexes and flip isomorphisms.

We begin by defining the relevant surfaces.  Let $\cylinder_n$ denote the infinite cylinder $(\R/n\Z)\times \R$ with a marked point at each integer lattice point. We think of this as a vertical strip of width $n$ in the plane with opposite sides identified. Let $\cylinder_n[m]$ denote the cylinder arising from the same strip where we apply a vertical shift of size $m$ when identifying the opposite edges of the strip; in other words, $\cylinder_n[m]$ is $\R^2 / \langle n, m \rangle$. We interpret $\cylinder_n[m]$ as being constructed .....

Let $\Gamma$ be a compact immersed multicurve in $\cylinder_n[m]$ and let $\bchain$ be a bounding chain for $\Gamma$. To extract a collection of bigraded complexes from $(\Gamma, \bchain)$, we will replace each marked point of $\cylinder_n[m]$ with a pair of marked points, with a $z$-marked point an infinitesimal distance to the left of the original marked point and a $w$-marked point and infinitesimal distance to the right. Note that the immersed curve $\Gamma$ was disjoint from the original marked points, and so we may assume that it is disjoint from the $z$ and $w$ marked points and does not pass between $z$ and $w$ for any pair. For each $i$ in $\Z/n\Z$, let $\mu_i$ denote the vertical line $x = i$ in $\cylinder_n[m]$; note that $\mu_i$ does pass between nearby $z$ and $w$ marked points. We now obtain a bigraded complex for each $i$ by taking the Floer homology of $(\Gamma, \bchain)$ with $\mu_i$. We equip $\mu_i$ with a trivial bounding chain

\begin{definition}
For a compact immersed multicurve $\Gamma$ in $\cylinder_n[m]$ decorated by a bounding chain $\bchain$, we define $C(\Gamma, \bchain; i)$ to be the bigraded complex $CF( (\mu_i, 0), (\Gamma, \bchain) )$.
\end{definition}

\begin{example}
Right hand trefoil curve.
\end{example}

\begin{example}

\end{example}

Given the cylinder $\cylinder_n[m]$, let $\mu_i$ denote the vertical line $x = i$ for each $i$ in $\Z/n\Z$. 



We claim that an immersed curve with a collection of turning points in the cylinder $\cylinder_n$ determines a co



-Define marked cylinder and punctured cylinder, define $\mu$ in doubly marked cylinder

-Each immersed multicurve with boundng chain in punctured cylinder determins a bigraded complex over $\sR$ by taking Floer homology with $\mu$.

-We can pertub curve so that no bigon intersects $x = \frac 1 2$. This means we can cut cylinder open to form strip, an immersed multicurve with bounding chain in the strip determines a bigraded complex

-An immersed multicurve with collection of left turn points $b$ determines a bigraded precomplex. We already have that if $b$ is a bounding chain then $d^2 = 0$. Show that the converse holds too.

-For an immersed curve with bounding chain in cylinder, we get a flip map from the complex to itself

-More generally, consider the width $n$ cylinder. We get $n$ different bigraded complexes, and flip maps connecting them.

-???: A non-bounding chain still determines a map. Bounding chain condition should correspond to the map being a chain map

-Point forward: It is not clear a priori that every bigraded complex can be represented this way. It is clear that every complex over $\sRhat$ can be represented this way, but we will show this can be done in a unique simple way

\section{Immersed curves and bounding cochains}

A primary goal of this paper is to encode bigraded chain complexes over $\sR$ in terms of geometric objects, namely immersed curves in certain surfaces decorated with a \emph{bounding cochain}. We will now introduce these objects and discuss their key properties, including a pairing from Floer homology. Floer theory for immersed Lagrangians with bounding cochains is developed in more generality in \cite{AkahoJoyce}, but we will focus on the case of curves in certain surfaces. In this special case, the theory can be defined combinatorially. Some technical results, needed to prove that the combinatorial construction in this section is well-defined, will be deferred to the Appendix.

\subsection{Immersed multicurves in the infinite strip and cylinder}

We will restrict our attention to immersed Lagrangians in either the \emph{infinite marked strip} or the \emph{infinite marked cylinder}. The infinite marked strip is defined to be
$$\strip = \left[-\tfrac 1 2, \tfrac 1 2\right]\times\R$$
equipped with two infinite families $\{z_n\}$ and $\{w_n\}$ of marked points, with $z_n$ occurring at the point $\left(-\epsilon, n - \tfrac 1 2\right)$ and $w_n$ occurring at the point $\left(+\epsilon, n - \tfrac 1 2\right)$ for some small $\epsilon$ and each integer $n$. We will sometimes refer to the punctured surface $\strip^\circ$ obtained by replacing the marked points $w_n$ and $z_n$ with a puncture at $\left(0, n - \tfrac 1 2\right)$ for each integer $n$. The infinite marked cylinder $\cylinder$ is obtained from $\strip$ by identifying the opposite boundaries, and the infinite punctured cylinder $\cylinder^\circ$ is obtained from $\strip^\circ$ in the same way.

An immersed Lagrangian in $\strip$ or $\cylinder$ is a collection of immersions $C \looparrowright \strip$ that avoid all basepoints, where $C$ is either $S^1$, $[0,1]$, $\R_{\ge 0}$, or $\R$, closed ends of intervals map to the boundary of $\strip$, and open ends of intervals approach one of the infinite ends of $\strip$ or $\cylinder$. A component with $C = S^1$ will be called an \emph{immersed curve} and a component with $C = [0,1]$ will be called an \emph{immersed arc} (note that immersed arcs do not occur in $\cylinder$). By slight abuse, we will sometimes use these terms to refer to the images of the immersion rather than the immersions themselves, but we believe the proper meaning will be clear. We will not consider components with $C = \R_{\ge0}$, and we will rarely allow $C$ to be $\R$. An important exception is the vertical line $\{0\}\times \R$ in $\strip$, which will play a special role; this line will be denoted $\mu$. Apart from $\mu$, unless otherwise noted, we assume all immersed Lagrangians are compact and thus consist of a collection of immersed curves and immersed arcs. Such a collection of immersed curves and arcs will also be called and \emph{immersed multicurve}. We will furthermore assume that, unlike $\mu$, immersed curves and arcs do not pass in between the two marked points at a given height.

Because immersed multicurves do not pass between pairs of marked points, these multicurves in the marked surfaces $\strip$ and $\cylinder$ give rise to immersed multicurves in the corresponding punctured surfaces $\strip^\circ$ and $\cylinder^\circ$ (in contrast, in these surfaces $\mu$ breaks into lines segments connecting adjacent punctures). With some caveats that will be discussed later, we will be interested in immersed multicurves only up to homotopy in the punctured surfaces $\strip^\circ$ and $\cylinder^\circ$; equivalently, we will allow homotopies of curves in the marked surfaces which are disjoint from all marked points, but we will not consider homotopies which pass over marked points.

The surfaces $\strip$ and $\cylinder$ will be called \emph{doubly marked} because they have two families of marked points. Immersed Lagrangians in a doubly marked surface define a curved $\Ainfty$ category with coefficients in the ring $\sR = \F[U,V\}$ as follows. Given two Lagrangians $L_0$ and $L_1$ with transverse intersection, we define $CF(L_0, L_1)$ to be the $\sR$-module generated by intersection points of $L_0$ and $L_1$. For $k \ge 0$ and each collection of immersed Lagrangians $L_0, \ldots, L_k$ such that each pair has transverse intersection, we define a map
$$m_k: CF(L_{k-1}, L_k) \otimes \cdots \otimes CF(L_0, L_1) \to CF(L_0, L_k)$$
by counting immersed $(k+1)$-gons. 

The infinite marked cylinder $\cylinder = S^1 \times \R$ is obtained from $\strip$ by identifying the two

 An immersion with $C = \S^1$ will be called an 

The vertical line $\{0\}\times\R$ in $\strip$ will be denoted by $\mu$; this particular non-compact Lagrangian will play a special role. Apart from $\mu$, unless otherwise noted, we will assume that all curves are compact and do not pass between the two marked points at a given height. 



Compact immersed Lagrangians in $\strip$ are collections of immersions $S^1 \looparrowright \strip$ and $[0,1] \looparrowright \strip$ which avoid all the marked points; the former are referred to as immersed curves and the latter are referred to as immersed arcs. Note that the endpoints of 

We will sometimes refer to the punctured surface $\strip^\circ$ obtained by replacing the marked points $w_n$ and $z_n$ with a puncture at $\left(0, n - \tfrac 1 2\right)$ for each integer $n$ . Note that in $\strip^\circ$, $\mu$ breaks into a collection of line segments connecting adjacent punctures, but all other curves are unaffected. Compact 


\subsection{Curved $\Ainfty$-category of immersed curves}

The category of immersed curves. 
The category of immersed curves decorated with turning points in a given surface forms an $\Ainfty$ category





